Latent Multimodal Functional Graphical Model Estimation

Joint multimodal functional data acquisition, where functional data from multiple modes are measured simultaneously from the same subject, has emerged as an exciting modern approach enabled by recent engineering breakthroughs in the neurological and biological sciences. One prominent motivation to acquire such data is to enable new discoveries of the underlying connectivity by combining multimodal signals. Despite the scientific interest, there remains a gap in principled statistical methods for estimating the graph underlying multimodal functional data. To this end, we propose a new integrative framework that models the data generation process and identifies operators mapping from the observation space to the latent space. We then develop an estimator that simultaneously estimates the transformation operators and the latent graph. This estimator is based on the partial correlation operator, which we rigorously extend from the multivariate to the functional setting. Our procedure is provably efficient, with the estimator converging to a stationary point with quantifiable statistical error. Furthermore, we show recovery of the latent graph under mild conditions. Our work is applied to analyze simultaneously acquired multimodal brain imaging data where the graph indicates functional connectivity of the brain. We present simulation and empirical results that support the benefits of joint estimation.

==> main/1_latent.tex <==
\section{The latent space structure}
In this manuscript, we study the functional data in the random element perspective, as compared to the mean-squared integrable stochastic processes perspective commonly studied in the functional graphical models. 
%Oftentimes, one could find a congruence mapping between two perspectives, i.e., the mean-squared integrable stochastic process perspective and the random element perspective, under mild assumptions of the Hilbert space $\HH$. Here, we take the random element viewpoint for mathematical conciseness.

Consider a p-dimensional mean-zero Gaussian random function vector in the latent space $\chi_z=(\chi_{z,1},\ldots,\chi_{z,p})\in\HH^p$, where $\HH$ is a separable Hilbert space of continuous functions defined on a closed interval $\mathcal{T}\subseteq \mathbb{R}$. Define $\dotp{\chi_{2}}{\chi_{1}}_{\HH^p}=\sum_{i=1}^p\dotp{\chi_{1,i}}{\chi_{2,i}}_{\HH}$. We see that $\chi_z:(\Omega,\Fcal,\PP)\rightarrow(\HH^p,\dotp{\cdot}{\cdot}_{\HH^p})$ is a random element taking values in the Hilbert space $\HH^p$. 
 %Define $\bar\chi_z=p^{-1}\sum_{i=1}^p\chi_{z,i}$ whose associated covariance operator is $\Kscr_{\bar z}$. By Theorem 7.2.6 in~\citep{hsing2015theoretical}, $\Kscr_{\bar z}$ admits the eigen decomposition $\Kscr_{\bar z}=\sum_{j=1}^\infty \lambda_{z,j}\phi_{z,j}\otimes \phi_{z,j}$, where 
We let $\{\phi_{z,1},\phi_{z,2}\ldots\}$ be a CONS for $\HH$.
For each $\chi_{z,i}$, $\pseq$,
the distribution of $\chi_{z,i}$ is uniquely defined by the marginal distribution $\dotp{ \chi_{z,i}}{\phi_{z,\ell}}_{\HH}$ for $\ell\in\NN\backslash\{0\}$ by Theorem 7.1.2 in~\citep{hsing2015theoretical}.
Noting that, in the random element perspective, we could make analogy the random function $X_{z,i}(\omega)\in\HH$ as an infinite dimensional random vector whose entries take values in $\RR$, denoted as $(\dotp{X_{z,i}}{\phi_{z,1}},\dotp{X_{z,i}}{\phi_{z,2}},\ldots)$. 
We then can represent the random element uniquely as
 \begin{equation}\label{eq:randomelement_p}
 \chi_{z,i}(\omega)=\sum_{\ell=1}^\infty z_{i,\ell}(\omega)\phi_{z,\ell},\qquad \omega\in\Omega,
 \end{equation}
 where $z_{i,\ell}(\omega)=\dotp{ \chi_{z,i}(\omega)}{\phi_{z,\ell}}_{\HH} \in \mathbb{R}$ is a Gaussian random variable taking values in $\RR$ and $\phi_{z,\ell} \in \mathbb{H}_z$ for $\ell\in\NN\backslash\{0\}$. The realization of~\eqref{eq:randomelement_p} at time $t\in\Tcal$ is hence
 \begin{align}\label{eq:stochaticprocess_p}
  \chi_{z,i}(\omega, t)=\sum_{\ell=1}^\infty z_{i,\ell}(\omega)\phi_{z,\ell}(t),\qquad \omega\in\Omega, t\in\Tcal.
 \end{align}
 
Due to the Gaussian assumption of the latent functions, the set of random variables $\chi_{z,1},\ldots,\chi_{z,p}$ is linearly dependent and has the following relationship:
 \[
 \chi_{z,i}=\sum_{j\in[p]\backslash \{i\}}\beta_{ij}^\star(\chi_{z,j})+\Wcal_i,
 \]
 where $\beta_{ij}^\star\in\bophs{\HH}{\HH}$ for $\pseq$ and $j\in[p]\backslash \{i\}$ is a function-on-function regression operator
 \[
\beta_{ij}^\star=\sum_{\ell,\ell'=1}^\infty b_{ij,\ell\ell'}^\star \phi_{z,\ell} \otimes \phi_{z,\ell'},\quad \pseq,\;j\in\pni,
 \] 
 and $\Wcal_i\in\HH$ is a Gaussian random function independent of $\chi_{z,j}$ for $j\in\pni$. 
 %\marginnote{\footnotesize What is the form of a normally distributed random vector taking values in $\HH^p$?}
 

 Therefore, for $\pseq$ and $j\in\pni$, we can write
 \[
 \beta_{ij}^\star(\chi_{z,j})=\sum_{\ell=1}^\infty\sum_{\ell'=1}^\infty
 b_{ij,\ell\ell'}^\star 
 \langle
\phi_{z,\ell'},\chi_{z,j}\rangle_{\HH}
 \phi_{z,\ell}.
 \]
 %Or equivalently, in the stochastic process perspective, we can represent it as
 In the high-dimensional setting, where $p$ is larger then the number of sample size $N$, we often consider that the coefficients are sparse -- many of $\beta_{ij}^\star$ are zero operators. Here, we assume that the set of coefficient functions $\{\beta_{ij}^\star\}_{j\in\pni}$ is $s^\star$-sparse. Hence, $\chi_{z,j}$ for $j\neq i$ is a neighbour of $\chi_{z,i}$ if $\beta_{ij}^\star$ is not a zero operator. Hence, the set of neighbor of $\chi_{z,i}$  is defined as \begin{align}\label{eq:def_pNi}
\pNi = \{j\in\pni:\norm{\beta_{ij}^\star}_{HS}>0\},    
\end{align}
and we have $\abr{\pNi}\leq s^\star$. Consequently, given $p$ latent nodes $V_z=\{\chi_{z,1},\ldots, \chi_{z,p}\}$, the underlying graph is defined as $\Gcal=(V_z, E_z)$
\[
E_z=\{(i,j):\norm{\beta_{ij}^\star}_{HS}>0 \text{ and } \norm{\beta_{ji}^\star}_{HS}>0,i\neq j\}.
\]

%The set of matrices $\defsetpBi$ for $i=1\ldots,p$ are sparse: most $\Bb_{ij}^\star$ are zero matrix. We assume that $\{\Bb_{i1}^\star,\ldots,\Bb_{ip}^\star\}$ are $s^\star$-group sparse, where at most $s^\star$ elements in the set $\{\Bb_{i1}^\star,\ldots,\Bb_{ip}^\star\}$ are nonzero.

Our model could be applied to estimate the conditional independence of dynamic brain networks, where we formulate the dynamic brain networks as stochastic processes. At each brain parcellation, $\chi_{z,i}(\omega,t)$ could be viewed as a random function of time $t\in\Tcal$. 

==> main/2_observation.tex <==

\section{The observation space}
  %Define $\bar\chi_{m}=p^{-1}\sum_{i=1}^p\chi_{m,i}$ whose corresponding covariance operator is $\Kscr_{\bar m}=\EE(\bar{\chi}_m\otimes\bar{\chi}_m)$. The covariance operator $\Kscr_{\bar{m}}$ admits an eigendecomposition
 %\begin{align}\label{eq:eigenKscrm}
 %    \Kscr_{\bar m} = \sum_{\ell=1}^\infty\lambda_{m,\ell}\phi_{m,\ell},
 %\end{align}
 %where $x_{i,l} \in \mathbb{R}$ and $\phi_{m,l} \in \mathbb{H}_z$.
 

 Given the underlying latent process $  \chi_z$, we that we have $M$ modalities of observations.
 For modality $m$, we observe data $\Ycal_m=(\Ycal_{m,1},\ldots,\Ycal_{m,p})^\top\in\HH_m^p$ and $\Ycal_{m,i}=\chi_{m,i}+\xi_{m,i}$ for $\pseq$. Here $\chi_{m,i}$ is a deterministic element given $\chi_{z,i}$, represented as  $\chi_{m,i}=\Lscr_m\chi_{z,i}$ ($\chi_{m,i}(t)=\int_{s\in\Tcal} \Lscr_m(s,t)\chi_{z,i}(s) ds$) for some bounded operator $\Lscr_m\in\mathfrak{B}(\HH,\HH_m)$, and $\xi_{m,i}$ is the additive noise or nuisance factor that are not shared across different modalities:  
 \[
 \Ycal_{m,i}=\chi_{m,i} + {\xi}_{m,i},\qquad
 \mseq,\;\pseq,
 \]
 where ${\xi}_{m,i}$ is a zero mean normally distributed random element with covariance operator $\Kscr_{m,i}^q$ and is independent of $\chi_{m,i}$. Define the covariance operator for $\chi_{m,i}$ for $\mseq$ and $\pseq$ as $\Kscr_{m,i}^x$, we then define $\Kscr_{m,i}= \Kscr_{m,i}^x + \Kscr_{m,i}^q$ be the covariance operator of $ \Ycal_{m,i}$.
 
 Here, $\{\phi_{m,1},\phi_{m,2},\ldots\}$ is a set of basis functions that constructs $\HH_m$. In addition, let
 \[
 \chi_{m,i}=\sum_{\ell=1}^\infty x_{m,i,\ell} \phi_{m,\ell}, \qquad \pseq.
 \]
 \section{Problem Formulation}
 Our problem is to study the graphical model in the latent space through data from multiple view. The fundamental challenge is that different modalities have different representations of the latent element, which are transformed by the operator $\Lscr_m$ for $\mseq$. Unfortunately, the forward operators $\Lscr_m$ are generally unknown. From the estimation procedure, however,  our goal is not to estimate the forward operator but to find the (pseudo) inverse operator of $\Lscr_m$, denoted as $\Ascr_m$, that maps the random element from the observation space back to the latent space. Then, we can estimate the shared latent graph.
 Such procedure, is commonly carried out by canonical correlation estimator, which finds the transformation of two random element that maximize the canonical correlation. Therefore, we define $\Ascr_m$ operator that maps from the observation space $\HH_m$ to the latent $\HH$: $\Ascr_m  \in  \bophs{\HH_m}{\HH}$, such that for every $\pseq$ and $\chi_{1,i},\ldots,\chi_{M,i}$, that are in the closure of the range space of $\overline{Im(\Lscr_m)}$, we have the following relationship
 \[
 \chi_{z,i}=\Ascr_m(\chi_{m,i}),\qquad \mseq.
 \]
 We assume $\Ascr_m$ has the form
 \[
 \Ascr_m =\sum_{\ell=1}^\infty\sum_{\ell'=1}^{\infty} a_{m,\ell\ell'}^\star  \phi_{z,\ell} \otimes \phi_{m,\ell'} .
 \]
 
 Thus for every $\chi\in\HH_m$, we have
\[
\Ascr_m(\chi)=\sum_{\ell=1}^\infty\sum_{\ell'=1}^{\infty} a_{m,\ell\ell'}^\star\langle  \phi_{m,\ell'},\chi\rangle \phi_{z,\ell}.
\]
 Thus the real valued sequence $\{a_{m,\ell\ell'}^\star\}_{\ell\ell' \geq 1}$ uniquely defines the operator $\Ascr_m$.
%  Moreover, we assume that for every $\pseq$ and $\chi_i^{1},\ldots,\chi_{m,i},\ldots,\chi_{m,i}$, we have the following relationship
%  \[
%  \chi_{z,i}=\Ascr_m(\chi_{m,i}),\quad \forall m\in[M].
%  \]
 
How does $\Lscr_m$ relates to $\Ascr_m$? If $\Lscr_m\in\bophs{\HH}{\HH_m}$, then the inverse operator does not exist because the spectrum of $\Lscr_m$ must contain zero eigenvalues. Hence, the pseudo-inverse of $\Lscr_m$, denoted as $\Lscr_m^\dagger$, is equal to $\Ascr_m$ restricted on the domain $\overline{Im(\Lscr_m)}$ and $0$ on the domain $\overline{Im(\Lscr_m)}^\perp$. That is, $\chi=\Lscr_m\Ascr_m\chi$ only if $\chi\in\overline{Im(\Lscr_m)}$. 
 
 
 %As a consequence of circumventing making assumptions on the forward operator, we directly formulate the relation in terms of the inverse operator.
 %\begin{remark}
 %We can look at $\Ascr_m$ for $\mseq$ as the linear operators that transform data from different Hilbert spaces to the same Hilbert space. A naive estimation procedure is to find operators that maximize the correlation of two projected random elements, which is also known as canonical correlation analysis (CCA). In the multivariate Gaussian data case, \citet{bach2005probabilistic}  has shown the relation of probabilistic CCA and a latent variable model. Such connection also exist in the functional data, as revealed in Section~\ref{sec:reasoning}.
 %\end{remark}



==> main/3_finite_dimensional.tex <==
%\section{Finite Dimensional Approximation}
In reality, due to the computational complexity, the estimation procedure works on the truncated finite dimensional space: we define the $k$-dimensional approximation of $\chi_{z,i}$ as
 \[
 \chi_{z,i}^{k}:=\sum_{\ell=1}^kz_{i,\ell}\phi_{z,\ell}\quad\pseq.
 \]
 %Therefore, for $\pseq$ and $j\in\pni$, we can write
 %\[
 %\beta_{ij}^\star(\chi_z_j^k)=\sum_{\ell=1}^\infty\sum_{\ell'=1}^\infty\langle b_{ij,\ell\ell'}^\star\phi_{\ell'}^0,\chi_z_j^k\rangle\phi_{\ell}^0
 %=\sum_{\ell=1}^\infty\sum_{\ell'=1}^k\langle b_{ij,\ell\ell'}^\star\phi_{\ell'}^0,\chi_z_j^k\rangle\phi_{\ell}^0,
 %\]
Similarly, We define the truncation of $\beta_{ij}^\star$ for $\pseq$ and $j\in\pni$ and $\chi_z\in\HH$ as
 \[
    \beta_{ij}^{\star k}(\chi_z)=\sum_{\ell=1}^k\sum_{\ell'=1}^k b_{ij,\ell\ell'}^\star \langle  \phi_{z, \ell'},\chi_z\rangle \phi_{z,\ell}.
 \]
Then, we can represent the truncated $\zb_i=(z_{i1},\ldots,z_{ik})^\top\in\RR^k$ from the infinite dimensional vector $(z_{i1},z_{i2},\ldots)$ in the following form
  \begin{align*}
 \zb_i&=\begin{pmatrix}z_{i1}\\\vdots\\z_{ik}\end{pmatrix}=\sum_{j\in[p]\backslash \{i\}}\underbrace{\begin{pmatrix}b_{ij11}^\star&\ldots&b_{ij1k}^\star\\&\ddots&\\b_{ijk1}^\star&\ldots&b_{ijkk}^\star\end{pmatrix}}_{\pBijk}\underbrace{\begin{pmatrix}z_{j1}\\\vdots\\z_{jk}\end{pmatrix}}_{\zb_j}
 +\rb_i+\wb_i=\sum_{j\in[p]\backslash \{i\}}\pBijk\zb_j+\rb_i+\wb_i,
 \end{align*}
 where 
 \[
 r_{ij}=\sum_{j'\in\pni}\sum_{\ell=k+1}^\infty\dotp{b_{ij'j\ell}\phi_{z,\ell}}{\chi_{z, j'}}    
 ,\quad w_{ij}=\dotp{\Wcal_i}{\phi_{z,j}},\quad j=1,\ldots,k,\]
and $\rb_{i}=(r_{i1},\ldots,r_{ik})\in\RR$ denotes the residual vector. Let $\EE(\rb_i\rb_i^{\top})=\Sigmab_i^{\rb}$ and  $\EE(\wb_i\wb_i^{\top})=\Sigmab_i^{\wb}$ for $\pseq$.

A fundamental question is how should we choose $k$ such that the truncated subspace could output reasonably correct graph. Observe that $\norm{\beta_{ij}^\star}_{HS}=\norm{\beta_{ij}^\star-\beta_{ij}^{\star k}+\beta_{ij}^{\star k}}_{HS}\leq \norm{\beta_{ij}^\star-\beta_{ij}^{\star k}}_{HS}+\norm{\beta_{ij}^{\star k}}_{HS}$. 
Hence, if there exist a positive $\epsilon_0$ such that for all $j\in \pNi$, $\beta_{ij}^\star$ has magnitude $\norm{\beta_{ij}^\star}_{HS}\geq2\epsilon_0$,
then we can choose a $k$ such that $\norm{\beta_{ij}^{\star}-\beta_{ij}^{\star k}}_{HS}\leq\epsilon_0$,
we have $\norm{\beta_{ij}^k}_{HS}\geq\epsilon_0$ for all $j\in \pNi$. Using the fact that $\norm{\beta_{ij}^k}_{HS}=\norm{\pBijk}_F$, then the set defined in~\eqref{eq:def_pNi} is equivalent as
\begin{align}\label{eq:def_pNi2}
    \pNi = \{j\in\pni:\norm{\pBijk}_{F}>\epsilon_0\}.    
\end{align}
That being said, if $k$ is properly selected, then we have hope to correctly recover $\pNi$ even though we're working on the finite-dimensional space. The assumption will be formally introduced in Assumption~\ref{assumption:edge_recovary}.

%The set of matrices $\defsetpBi$ for $i=1\ldots,p$ are sparse: most $\Bb_{ij}^\star$ are zero matrix. We assume that $\{\Bb_{i1}^\star,\ldots,\Bb_{ip}^\star\}$ are $s^\star$-group sparse, where at most $s^\star$ elements in the set $\{\Bb_{i1}^\star,\ldots,\Bb_{ip}^\star\}$ are nonzero.

We define the finite approximation in the observation space as
 \[
 \chi_{m,i}^{k_m}:=\sum_{\ell=1}^{k_m}x_{m,i,\ell} \phi_{m,\ell},\quad\pseq,\mseq.
 \]

 Then, we can write
 \begin{align}\label{eq:z_A}
 \chi^{k}_{z,i} = \sum_{\ell=1}^k\dotp{\Ascr_m(\chi_{m,i})}{\phi_{z,\ell}}\phi_{z,\ell} 
 &=\sum_{\ell'=1}^\infty
 \sum_{\ell=1}^k
 \dotp{a_{m,\ell\ell'}^\star \phi_{m,\ell'}}{\chi_{m,i}}\phi_{z,\ell}\notag\\
 &=  \sum_{\ell'=1}^{k_m}
 \sum_{\ell=1}^k
 \dotp{a_{m,\ell\ell'}^\star \phi_{m,\ell'}}{\chi_{m,i}}\phi_{z,\ell}
 +\sum_{\ell'=k_m+1}^\infty
 \sum_{\ell=1}^k
 \dotp{a_{m,\ell\ell'}^\star
 \phi_{m,\ell'}}{\chi_{m,i}}\phi_{z,\ell}.
 \end{align}
If $k_m$ is selected to be large enough, the second term would be negligible. To simplify the analysis, we assume that the second term is $0$. Then, Equation~\eqref{eq:z_A} has following equivalent expression in the matrix form
 \[
 \zb_i
 =
 \begin{pmatrix}
 z_{i1}\\\vdots\\z_{ik}
 \end{pmatrix}
 =
 \underbrace{
    \begin{pmatrix}
        a_{m,11}^\star&\ldots& a_{m,1k_m}^\star\\
        &\ddots&\\
        a_{m,k_m1}^\star&\ldots&a_{m,k_mk_m}^\star
    \end{pmatrix}
    }_{\pAmk}
    \underbrace{
        \begin{pmatrix}
        x_{m,i1}\\\vdots\\x_{m, ik_m}\end{pmatrix}
    }_{\xkmfree{i}}=\pAmk \xkmfree{i}. %+\ub_{m,i},
 \]
 %where 
 %\[
 %u_{m,i,j}
 %=
 %\sum_{\ell'=k_m+1}^\infty\dotp{a_{m, j\ell'}^\star
 %\phi_{m,\ell'}}{\chi_{m,i}}
 %,\quad j=1,\ldots,k,    
 %\]
 %and $\ub_{m,i}=(u_{m,i,1},\ldots,u_{m,i,k})^\top\in\RR^k$ is the truncation error. 
 %Let $\ub_m=(\ub_{m,1}^{\top},\ldots,\ub_{m,p}^{\top})^\top\in\RR^{kp}$ and $\EE(\ub_m\ub_m^{\top})=\Sigmab^{\ub}_m$. 
 
 Combining everything together, we then have the relationship
\begin{equation}\label{eq:neighbour_reg}
    \pAmk \xkmfree{i} = \sum_{j\in\pni}\pBijk\pAmk \xkmfree{j}+\rb_i+\wb_i,
\end{equation}
  where $\wb_i$ follows independently from $\Ncal({\bf 0},\Sigmab^{\wb}_i)$. 
Then, let ${\qb}_{m,i}=(e_{m,i,1},\ldots,e_{m,i,k_m})^\top$ where $e_{m,i,j}=\dotp{\xi_{m,i}}{\phi_{m,j}}$ for $j=1,\ldots k_m$, we define the finite truncation of the observed random vector as
\begin{equation}\label{eq:observation}
\yb_{m,i} = \xb_{m,i} + \qb_{m,i},\qquad\mseq,\pseq,
\end{equation}
where $\qb_{m,i}$ is the noise in the observation space and follows distribution $\Ncal({\bf 0}, \Sigmab^{m,\qb}_i)$
 
 
 
 
 
 
 %Let $\Ykmnfree{i}=(\xkmnfree{i}{1},\ldots, \xkmnfree{i}{N})\in\RR^{k_m\times N}$ be a matrix whose columns are independent copies of $\xkmfree{i}$ for $\pseq$ and $\mseq$. Here, for simplicity of the analysis, we assume that each modality has $N$ independent samples. 
 %We have the following relationship
 %\[
 %\pAmk \Xkmnfree{i}
 %=
 %\sum_{j\in\pni}\pBijk\pAmk \Xkmnfree{j}+\sum_{j\in\pni}\pBijk\Ub_{m,j}^{k, N}-\Ub_{m,i}^{k, N}+\Rb_i^{k, N}+\Wb_i^{k, N},
 %\]

 

==> main/4_basis_estimation.tex <==
\section{Estimation of basis functions}
%introduce \hat x.
We apply functional PCA to estimate the basis for each $\HH_m$. Recall that $\bar\chi_m=p^{-1}\sum_{i=1}^p\chi_{m,i}$ and $\Kscr_{ m}=\EE(\bar\chi_m\otimes\bar\chi_m)$. We define the empirical estimator $\hat\Kscr_{\bar m}=N^{-1}\sum_{n=1}^N\bar\chi_m^{(n)}\otimes \bar\chi_m^{(n)}$ with associated eigen system $\{(\hat\lambda_{m,j},\hat{\phi}_{m,j})\}$ for $\mseq$. Consequently, we take $\{\hat{\phi}_{m,1},\hat{\phi}_{m,2},\ldots\}$ for the estimated principal basis for $\HH_m$ for $\mseq$. Furthermore, we denote
$\hxkmnfree{i}
=
(
\dotp{\chi_{m,i}^{(n)}}{\hat{\phi}_{m,1}},
\ldots, 
\dotp{\chi_{m,i}^{(n)}}{\hat{\phi}_{m,k_m}})^\top
\in\RR^{k_m}$ for $\mseq$, $\pseq$ and $\nseq$. We denote $\hxkmn{n}
=
(\hxkmnfreeT{1}
,\ldots,
\hxkmnfreeT{p})^\top\in\RR^{pk_m}$,
$\hXkmn
=
(
\hxkmn{1},\ldots,\hxkmn{N})\in\RR^{pk_m\times N}$, and $\hsCov=N^{-1}\hXkmn(\hXkmn)^\top$.

%Here, we define $\varepsilon_N:=\max\cbr{\norm{\hat\Kscr_{\bar 1} - {\Kscr}_{\bar 1}},
%\norm{\hat\Kscr_{\bar 2} - {\Kscr}_{\bar 2}},
%\norm{\hat\Kscr_{\bar{1}\bar{2}} - \Kscr_{\bar{1}\bar{2}}}}$ and
%$\delta_{k_1,k_2}:=\norm{\Cscr_{12}^{k_1,k_2}-\Cscr_{12}}$. 
%In the dense sampling setting, by central limit theorem, we have $\varepsilon_N=O(N^{-1/2})$. 
Recall the definition of $\lambda_{m,\ell}$ for $\mseq$, $\ell\in\NN$ in~\eqref{eq:eigenKscrm}., we define the eigengap to be
\[
\zeta_{m,j}=\frac{1}{2}\inf_{s\neq j}|\lambda_{m,j}-\lambda_{m,s}|,\quad \zeta_m^{k} = \min_{j\leq k}\zeta_{m,j},\quad \mseq.
\]
We make following assumptions.
\begin{assumption}\label{assumption1}
     $\Kscr_{\bar{m}}$ for $\mseq$ have distinct eigenvalues.
\end{assumption}
This ensures that $\zeta_{m,j}$ is always bounded away from zero. I think this assumption is general in perturbation analysis and the estimation error is proportional on the inverse of $\zeta_{m,j}$.\footnote{The introduction of Assumption~\ref{assumption1} seems out of place, move it to appropriate section.}

==> main/7_initialization_error.tex <==

%\subsection{temporary assumptions}
%\begin{assumption}
%Assume that $\Kscr_{m,i}=\Kscr_{m,i'}$ for $i\neq i'$ and $\mseq$. 
%\end{assumption}

%This assumption implies that $\Kscr_{z,i}=\Kscr_{z,i'}$ for $i\neq i'$. \\
%{\bf discussion}:
%Here, to solve the identifiability problem in canonical correlation,
%we need to assume that $\chi_{z,i}$ is from a Gaussian distribution with $\Kscr_{z,i}$ being an identity operator. (At least this is how people do it in the finite dimensional case) However, if we assume that $\Kscr_{z,i}$ for $\pseq$ is an identity operator, it will cause trouble. This is because, in infinite dimensional space, an identity operator is not compact, while both $\Kscr_{m,i}$ and $\Ascr_m$ is compact. On the other hand, the composite of compact operators $\Ascr_m\Kscr_{m,i}\Ascr_m=\Kscr_{z,i}$ should be compact and hence contradicts. 

\subsection{Introduction}


For simplicity, we assume that $M=2$. 
We define $\Bar\chi_m = p^{-1}\sum_{i=1}^p\chi_{m,i}\in\HH_m$ and the corresponding covariance operator to be ${\Kscr}_{\bar m}=\EE[\bar\chi_m \otimes \bar\chi_m]$. We define $\{\lambda_{m,j},e_{m,j}\}_{j=1}^\infty$ be the eigensystem of ${\Kscr}_{\bar m}$ for $m=1,2$ and $\{\lambda_{z, j},e_{z,j}\}_{j=1}^\infty$ be the eigensystem of the latent covariance operator $\Kscr_z$. $\{\lambda_{z,j},e_{z,j}\}_{j=1}^\infty$ is a set of abstract objects that helps us lay out the mathematical foundation of our optimization problem but we do not estimate them. We denote $\GG(\Kscr)$ be the Hilbert space generated by the covariance operator $\Kscr=\sum_{j=1}^\infty\lambda_je_j\otimes e_j$:
\[
\GG(\Kscr) = \cbr{f:\sum_{j=1}^\infty \lambda_j(\dotp{f,e_j})^2<\infty},
\]
associated with inner product defined as $\dotp{f}{g}_{\GG(\Kscr)}=\sum_{j=1}^\infty\lambda_j \dotp{f}{e_j}\dotp{g}{e_j}$ for $f,g\in\GG(\Kscr)$. 
In the following, for notation simplicity, we define $\GG_{\bar 1}=\GG(\Kscr_{\bar 1})$, $\GG_{\bar 2}=\GG(\Kscr_{\bar 2})$, and
$\GG_{\bar z}=\GG(\Kscr_{\bar z})$.

Recall the definition of the projection operator $\Ascr_m:\HH_m\rightarrow \HH_z$:
\[
\Ascr_m
=
\sum_{\ell=1}^\infty \sum_{\ell'=1}^\infty 
{a}_{m,\ell\ell'}
e_{z,\ell} \otimes e_{m,\ell'} ,\quad \sum_{\ell=1}^\infty \sum_{\ell'=1}^\infty\abr{{a}_{m,\ell\ell'}}^2<\infty.
\]
By linearity property of Hilbert-Schmidt operator, we observe that
\begin{equation}\label{eq:relationz}
\Ascr_m\bar\chi_m 
= 
\frac{1}{p}\sum_{i=1}^p\Ascr_m\bar\chi_{m,i}
= \frac{1}{p}\sum_{i=1}^p\chi_{z,i}=:\bar\chi_z,\quad m=1,2.
\end{equation}
Let $\rho_{\bar{z}}:\HH_z\times \HH_z\rightarrow\RR$ be the correlation functional defined as
\[
    \rho_{\bar{z}}(f_1,f_2)
    =
    \frac{\Cov(\dotp{\bar\chi_z}{f_1}\dotp{\bar\chi_z}{f_2})}{\sqrt{
        \Var(\dotp{\bar\chi_z}{f_1})
        \Var(\dotp{\bar\chi_z}{f_2})
    }},
\]
where $f_1,f_2\in\GG_{\bar z}$. 
%and $f_1,f_2\in\Rcal(\Kscr_{\bar z}^{1/2})$, for $\Kscr_z$ being the covariance operator of $\bar\chi_z$. 

\begin{remark}
The condition that $f_1,f_2$ belong to $\GG_{\bar z}$ directly implies that (i) $\Var(\dotp{\bar\chi_z}{f_m})\neq 0$  for $f_m \neq 0$ and (ii) $\Var(\dotp{\bar\chi_z}{f_m})<\infty$ for $m=1,2$. Therefore, $\rho_z(f_1,f_2)$ is well-defined.
\end{remark}


Note that if $f=f_1=f_2$, then $\rho_{\bar{z}}(f_1,f_2)=1$. Then, we can plug~\eqref{eq:relationz} into the above and obtain
\begin{align*}
    \rho_z(f,f)
    & =
        \frac{\Cov(\dotp{\Ascr_1\bar\chi_1}{f}
            \dotp{\Ascr_1\bar\chi_2}{f})}{\sqrt{
            \Var(\dotp{\Ascr_1\bar\chi_1}{f})
            \Var(\dotp{\Ascr_2\bar\chi_2}{f})
        }}\\
    & =
        \frac{\Cov(\dotp{\bar\chi_1}{\Ascr_1^*f}
            \dotp{\bar\chi_2}{\Ascr_2^*f})}{\sqrt{
            \Var(\dotp{\bar\chi_1}{\Ascr_1^*f})
            \Var(\dotp{\bar\chi_2}{\Ascr_2^*f})
        }},
\end{align*} 
where $\Ascr_m^*$ is the adjoint operator of $\Ascr_m$ for $m=1,2$.

Since for any $f\in\GG_{\bar z}$, we must have $\rho_x(f,f)=1$, we can hence estimate $\Ascr_1$ and $\Ascr_2$ by maximizing the following objective function. 
\begin{align}\label{eq:correlation_p}
\argmax_{\substack{
g_1=\Ascr_1^* f\in\GG_{\bar 1},\;
\norm{g_1}_{\GG_{\bar 1}}=1\\
g_2=\Ascr_2^* f\in\GG_{\bar 2},\;
\norm{g_2}_{\GG_{\bar 2}}=1\\
f\in\GG_{\bar z},\;
\norm{f}_{\GG_{\bar z}}=1
}} 
\rho_{12}(g_1,g_2)
=
    \argmax_{\substack{
    g_1=\Ascr_1^* f\in\GG_{\bar 1},\;
    \norm{g_1}_{\GG_{\bar 1}}=1\\
    g_2=\Ascr_2^* f\in\GG_{\bar 2},\;
    \norm{g_2}_{\GG_{\bar 2}}=1\\
    f\in\GG_{\bar z},\; 
    \norm{f}_{\GG_{\bar z}}=1
    }} 
    \frac{
        \Cov(\dotp{\bar\chi_1}{g_1}
            \dotp{\bar\chi_2}{g_2}
        )}{\sqrt{
            \Var({\dotp{\bar\chi_1}{g_1}})
            \Var({\dotp{\bar\chi_2}{g_2}})
        }}.
\end{align}
Note that we do not need to explicitly pick a $f\in\GG_{\bar z}$ in order to solve the above objective function. Instead, $f$ is a proxy that helps us find the maximum projection of two Hilbert spaces. 

We find the first canonical variable by first picking a $f_{z,1}$ from $\{e_{z,1},e_{z,2},\ldots\}$ that maximize~\eqref{eq:correlation_p}. Without the loss generality, we denote $f_{z,1}=e_{z,1}$ and $f_{z,1}\in\GG_{\bar z}$ because $\norm{f_{z,1}}_{\GG_{\bar z}}^2=\lambda_{z,1}<\infty$. Plugging $f_{z,1}$ into~\eqref{eq:correlation_p}, we can see the problem as finding the the first pair of canonical variables
\[
    {g}_{1,1}^\star,{g}_{2,1}^\star=\argmax_{\substack{
    \norm{g_{1}}_{\GG_{\bar 1}}=1,\\
    \norm{g_{2}}_{\GG_{\bar 2}
    }=1
    }} 
    \frac{
        \Cov(\dotp{\bar\chi_1}{g_{1}}
            \dotp{\bar\chi_2}{g_{2}}
        )}{\sqrt{
            \Var({\dotp{\bar\chi_1}{g_{1}}})
            \Var({\dotp{\bar\chi_2}{g_{2}}})
        }}.
\]
As $f_{z,1}$ being fixed, ${g}_{1,1}^\star$ and ${g}_{2,1}^\star$ reveals the partial structure of $\Ascr_1$ and $\Ascr_2$: 
\begin{equation}\label{eq:ga}
{g}_{1,1}^\star
    =
    \Ascr_{1}^*f_{z,1}
    =
    \sum_{\ell'=1}^\infty a_{1,1\ell'}^{\star} e_{1,\ell'}
    ,\quad
{g}_{2,1}^\star
    =
    \Ascr_y^*e_{z1}
    =
    \sum_{\ell'=1}^\infty a_{2,1\ell'}^\star e_{2,\ell'},
\end{equation}
where we will formally formulate the relation in Proposition~\ref{prop:projP}.
Noting that the property of covariance operator leads to 
\[
\Cov(
\dotp{\bar\chi_z}{e_{z,\ell}}
\dotp{\bar\chi_z}{e_{z,\ell'}}
)
=
\dotp{e_{z,\ell}}{\Kscr_ze_{z,\ell'}}=0, \quad \ell\neq \ell'.
\]
Consequently, let $g_{m,\ell}=\Ascr_m^*e_{z,\ell'}$, we can rewrite the above equation with $\bar\chi_z=\Ascr_m\bar{\chi}_m$ as
\[
\Cov(
\dotp{\bar\chi_m}{g_{m,\ell}}
\dotp{\bar\chi_m}{g_{m,\ell'}}
)=0,\quad\ell\neq\ell'.
\]
Subsequently, we optimize the following function
\[
    ( g_{1,2}^\star, g_{2,2}^\star)=\argmax_{\substack{
    g_1=\Ascr_x^* f
    ,\;
    \norm{g_1}_{\GG_{\bar 1}}=1
    ,\;
    {
    \Cov(\dotp{\bar\chi_1}{g_{1,1}^\star},\dotp{\bar\chi_1}{g_1})=0
    };\\
    g_2=\Ascr_y^* f,\;
    \norm{g_2}_{\GG_{\bar 2}}=1
    ,\;
    {
    \Cov(\dotp{\bar\chi_2}{g_{2,1}^\star},\dotp{\bar\chi_2}{g_2})=0
    };\\
    f\in\GG_{\bar z},\;
    {
    \dotp{f_{z,1}}{f}=0
    }
    }} 
    \frac{
        \Cov(\dotp{\bar\chi_1}{g_1}
            \dotp{\bar\chi_2}{g_2}
        )}{\sqrt{
            \Var({\dotp{\bar\chi_1}{g_1}})
            \Var({\dotp{\bar\chi_2}{g_2}})
        }}.
\]
We can simplify the above equation by choosing $f_{z,2}=e_{z,2}$ and the resulting optimization problem is equivalent as finding the second pair of canonical variables:
\[
    (g_{1,2}^\star,g_{2,2}^\star)=\argmax_{\substack{
    \norm{g_1}_{\GG_{\bar 1}}=1,\;
    \Cov(\dotp{\bar\chi_1}{g_{1,1}^\star},\dotp{\bar\chi_1}{g_1})=0;\\
    \norm{g_2}_{\GG_{\bar 2}}=1,\;
    \Cov(
    \dotp{\bar\chi_2}{g_{2,1}^\star}
    \dotp{\bar\chi_2}{g_2})=0
    }} 
    \frac{
        \Cov(\dotp{\bar\chi_1}{g_1}
            \dotp{\bar\chi_2}{g_2}
        )}{\sqrt{
            \Var({\dotp{\bar\chi_1}{g_1}})
            \Var({\dotp{\bar\chi_2}{g_2}})
        }}.
\]
Then, we can iterate the above method for $k$ times to obtain $k$ pairs of canonical vectors: For every $f_{z,j}$, $j=1,\ldots,k$ we want to solve the problem:
\begin{equation}\label{eq:ccaproblem}
    (g_{1,j}^\star,g_{2,j}^\star)=\argmax_{\substack{
    \norm{g_1}_{\GG_{\bar 1}}=1,\;
    \Cov(\dotp{\bar\chi_1}{g_{1,\ell}^\star},\dotp{\bar\chi_1}{g_1})=0, \;\ell=1,\ldots,j-1;\\
    \norm{g_2}_{\GG_{\bar 2}}=1,\;
    \Cov(
    \dotp{\bar\chi_2}{g_{2,\ell}^\star}
    \dotp{\bar\chi_2}{g_2})=0
    , \;\ell=1,\ldots,j-1
    }} 
    \frac{
        \Cov(\dotp{\bar\chi_1}{g_1}
            \dotp{\bar\chi_2}{g_2}
        )}{\sqrt{
            \Var({\dotp{\bar\chi_1}{g_1}})
            \Var({\dotp{\bar\chi_2}{g_2}})
        }}.
\end{equation}

\begin{proposition}\label{prop:projP}
%properties of g
Given $m=1,2$, $i,j\in\NN$, we have $a_{i,j}^\star=\dotp{g_{m,i}^\star}{e_{m,j}}$.
\end{proposition}
\begin{proof} This is direct consequence of the generalization of~\eqref{eq:ga} and~\eqref{eq:ccaproblem}.
\end{proof}

We show that finding $(g_{1,j}^\star,g_{2,j}^\star)$ for $j\in\NN$ is equivalent as finding the singular system of a compact operator $\Cscr_{12}$ defined below.
\begin{theorem}\label{theorem:cca2svd} Let $\tilde{\phi}_{m,j}=\lambda_{m,j}^{-1/2}e_{m,j}$ for $m=1,2$ and $j\in\NN$. There exists a linear bounded operator $\Cscr_{12}\in\mathfrak{B}(\GG(\Kscr_{\bar1}), \GG(\Kscr_{\bar2}))$:
\[
\Cscr_{12}
=
\sum_{i,j=1}^\infty d_{ij}\tilde{\phi}_{1,i}\otimes\tilde{\phi}_{2,j},\quad 
d_{ij} = \Cov(
    \dotp{\bar\chi_1}{\tilde{\phi}_{1,i}}
    \dotp{\bar\chi_2}{\tilde{\phi}_{2,j}}
)\quad i,j\in\NN.
\]
Assume that $\Cscr_{12}$ is compact, then the associated $j$-th left and right singular functions is the solution to~\eqref{eq:ccaproblem} for $j\in\NN$.
\end{theorem}
\begin{remark}
Therefore, a naive estimation approach is to construct an empirical estimator of $\Cscr_{12}$ and find the associated empirical singular system to estimate $(g_{1,j}^\star, g_{2,j}^\star)$ for $j\in\NN$.
\end{remark}
\subsection{Initialization Procedure}
We discuss the construction of the empirical estimator $\hat\Cscr_{12}$. In reality, because of the computation limitation, we can only work on the finite dimensional space. Hence, we define the truncated operator $\Cscr_{12}^{k_1,k_2}:\GG(\Kscr_{\bar 2}^{k_2})\rightarrow\GG(\Kscr_{\bar 1}^{k_1})$ as
\[
\Cscr_{12}^{k_1,k_2} 
= 
\sum_{\ell=1}^{k_1}\sum_{\ell'=1}^{k_2}
d_{\ell\ell'}
\tilde{\phi}_{1,\ell}\otimes\tilde{\phi}_{2,\ell'}.
\]
Suppose that we can select $k_1$ and $k_2$ large enough such that $\norm{\Cscr_{12}^{k_1,k_2}-\Cscr_{12}}:=\delta_{k_1,k_2}$ is small.
A naive construction of the empirical estimator hence would be
\[
\hat{\Cscr}_{12}^{k_1,k_2} 
= 
\sum_{\ell=1}^{k_1}
\sum_{\ell'=1}^{k_2}
\hat{d}_{\ell\ell'}
\rbr{{\hat\lambda_{1,\ell}^{-1/2}}\hat e_{1,\ell}}
\otimes
\rbr{{\hat\lambda_{2,\ell'}^{-1/2}}\hat e_{2,\ell'}},
\]
where
\[
\hat d_{\ell\ell'} 
= 
\frac{1}{N}\sum_{n=1}^N
\left\langle{\bar\chi_1^{(n)}},
\frac{\hat{\phi}_{1,\ell}}{{\hat\lambda_{1,\ell}}^{1/2}}\right\rangle
\left\langle{\bar\chi_2^{(n)}},
\frac{\hat{\phi}_{2,\ell
}}{{\hat\lambda_{2,\ell'}}^{1/2}}\right\rangle.
\]

Define $\Db = (d_{\ell,\ell'})$ be the matrix whose $\ell,\ell'$-entry is $d_{\ell,\ell'}$ and the corresponding singular system to be $\{(\rho_j,\hat\ub_j,\hat\vb_j)\}_{j=1}^{(k_1 \wedge k_2)}$, then according to~\cite{hsing2015theoretical}, we can obtain $g_{m,j}$ for $m=1,2$ and $j=1,\ldots,k$ of the form


\begin{equation}\label{eq:ghat}
\hat{g}_{1,j}^{k_1}
=
\sum_{\ell=1}^{k_1}
\frac{\hat u_{j\ell}}{\hat\lambda_{1,\ell}^{1/2}}
\hat e_{1,\ell},
\quad
\hat{g}_{2,j}^{k_2} = 
\sum_{\ell=1}^{k_2}
\frac{\hat v_{j\ell}}{\hat\lambda_{2,\ell}^{1/2}}
\hat e_{2,\ell}.
\end{equation}


\begin{remark}\label{rmk:asymptoticbias}
Recall that $g_{m,\ell}^\star=\Ascr_me_{z,\ell}$ and let $g_{m,\ell}^{k_m\star}=\sum_{\ell=1}^{k_m}\dotp{g_{m,\ell}^\star}{e_{m,\ell}}e_{m,\ell}$ for $\ell=1,\ldots k$ and $m=1,2$. 
Although we have 
$
\Cov(
\dotp{\bar\chi_m}{g_{m,\ell}^\star}
\dotp{\bar\chi_m}{g_{m,\ell'}^\star}
)=0$ for $\ell\neq \ell'$, this does not guarantee that $
\Cov(
\dotp{\bar\chi_m}{g_{m,\ell}^{k_m\star}}
\dotp{\bar\chi_m}{g_{m,\ell'}^{k_m\star}}
)=0$. However, for any $N$, $\hat g_{m,\ell}^{k_m}$ estimated via singular decomposition will always satisfy 
$$N^{-1}\sum_{n=1}^N\dotp{\bar\chi_m^{(n)}}{\hat g_{m,\ell}^{k_m}}\dotp{\bar\chi_m^{(n)}}{\hat g_{m,\ell'}^{k_m}}=0.$$ 
Therefore, $ g_{m,\ell}^{k_m}$ does not converge to $g_{m,\ell}^\star$ for $m=1,2$. We will discuss how to quantify the asymptotic bias in the following section.
\end{remark}
Then, By projecting~\eqref{eq:ghat} to $\{\hat e_{1,1},\ldots,\hat e_{1,k_1}\}$ and $\{\hat e_{2,1},\ldots,\hat e_{2,k_2}\}$ respectively, we have
\[
\hat{\Ab}_{1}^{k_1} 
= 
\begin{pmatrix}
\frac{\hat u_{1,1}}{\hat\lambda_{1,1}^{1/2}}&
\ldots&
\frac{\hat u_{1,k_1}}{\hat\lambda_{1,k_1}^{1/2}}\\
&\ddots&\\
\frac{\hat u_{k,1}}{\hat\lambda_{1,1}^{1/2}}&
\ldots&
\frac{\hat u_{k,k_1}}{\hat\lambda_{1,k_1}^{1/2}}
\end{pmatrix},\quad
\hat{\Ab}_{2}^{k_2} 
= 
\begin{pmatrix}
\frac{\hat v_{2,1}}{\hat\lambda_{2,1}^{1/2}}&
\ldots&
\frac{\hat v_{2,k_2}}{\hat\lambda_{2,k_2}^{1/2}}\\
&\ddots&\\
\frac{\hat v_{k,1}}{\hat\lambda_{2,1}^{1/2}}&
\ldots&
\frac{\hat v_{k,k_2}}{\hat\lambda_{2,k_2}^{1/2}}
\end{pmatrix}.
\]

\subsubsection{Estimation of regression coefficients}
After obtaining $\hat\Ab_m^k$ for $m=1,2$, the next step is to compute the initial guess for $\{\Bb_i^k\}_{\pseq}$. We solve the following constrained optimization problem:
\[
        \min_{\setBk} h_{\hat\Ab}(\setBk)
        =
        \min_{\substack{\Bik\in\Kcal_B(s,\alpha);\\
        \pseq}}
        \sum_{i=1}^p\sum_{m=1}^M\frac{1}{2MN}
        \bignorm{
            \hat\Ab_m^k\hXkmnfree{i}  
            -
            \Bik\bigAd{p-1}{\hat\Ab_m^k}\hXkmnfree{\noi}
        }_F^2.
\]
We solve the above optimization problem via projected gradient descent as described in Algorithm~\ref{alg:initializationB}.


\begin{algorithm}[H]\label{alg:initializationB}
    \SetAlgoLined
    \KwResult{ $\{\hat\Bb_i^k\}_{\pseq}$ }
    \KwIn{$\{\hat\Ab_m^{k}\}_{\mseq}$}
     \While{Not converge}{
     \For{$\pseq$}{
     $\Bb_i^{k,(t+1)}\leftarrow \Tcal_{\gamma_1s^\star/2}(\Bb_i^{k,(t)} - \eta_B\nabla_{\Bb_i^k}h_n)$\;
     }
    }
    \caption{Initialization of $\{\Bb_i^k\}_{\pseq}$}
\end{algorithm}




\subsection{Analysis}
In this section, we discuss the initialization error induced by the estimation procedure. Here, we define $\varepsilon_N:=\max\cbr{\norm{\hat\Kscr_{\bar 1} - {\Kscr}_{\bar 1}},
\norm{\hat\Kscr_{\bar 2} - {\Kscr}_{\bar 2}},
\norm{\hat\Kscr_{\bar{1}\bar{2}} - \Kscr_{\bar{1}\bar{2}}}}$ and
$\delta_{k_1,k_2}:=\norm{\Cscr_{12}^{k_1,k_2}-\Cscr_{12}}$. 
In the dense sampling setting, by Lemma~\ref{lemma:Kscr_sample bound} , we have $\varepsilon_N=CN^{-1/2}$ for some constant $C>0$ with high probability. 

%Let $\hat\Xb_1=(\hat\xb_1^{(1)},\ldots,\hat\xb_i^{(n)})\in\RR^{k_1\times n}$,$\Xb_1^\star=(\xb_1^{(1)\star},\ldots,\xb_i^{(n)\star})\in\RR^{k_1\times n}$ and
%\[
%\xb_1^{(r)\star} = \begin{pmatrix}
%\dotp{\bar\chi_1^{(r)}}{e_{11n}}\\
%\vdots\\
%\dotp{\bar\chi_1^{(r)}}{e_{1k_1n}}\\

%\end{pmatrix},\quad 
%\hat\xb_1^{(r)} = \begin{pmatrix}
%\dotp{\bar\chi_1^{(r)}}{e_{11}}\\
%\vdots\\
%\dotp{\bar\chi_1^{(r)}}{e_{1k_1}}\\

%\end{pmatrix},
%\quad r=1,\ldots, n.
%\]


\begin{theorem}\label{theorem:iniA}
%initialization error for both A and B.
Under Assumption~\ref{assumption1} and $\min_{\mseq} k_m > k$. Let  $C_0,C_1$ be constants depending on eigenvalues of ${\Kscr}_{\bar 1}$ and ${\Kscr}_{\bar 2}$. For any $\delta>0$, if $\SCthree$, then
\begin{align*}
    \norm{\hat\Ab_1^k-\Ab_1^{k\star}}_F^2
    = C_1\frac{
    {
    k\delta_{k_1,k_2}^2
    +
    (k\vee k_1)
    +
    k(k_1^2(\zeta_1^{k_1})^{-2}\vee  k_2^2(\zeta_2^{k_2})^{-2})
    }
    }{N}, 
\end{align*}
with probability at least $1-3\delta$.
\end{theorem}

\subsubsection{Distance of regression coefficient}\label{sec:REC}



\begin{assumption}\label{assumption:km}
$k_m$ is selected large enough such that $\nu_x(8\sqrt{\rho_x k_m \norm{\Kscr_{m,i}}_2})^{-1}<1$ for $\mseq$.
\end{assumption}

\begin{lemma}\label{lemma:initial_stepB} Under Assumption~\ref{assumption1},\ref{assumption:km} and let $\delta_0=\{\max_{\mseq} k_m(s^\star+1)\vee k^2\log s^\star\}$ and $\delta_1>0$. Suppose that $\SCsix$, $\Bb_i^{k,(0)}={\bf 0}$ for $\pseq$.
    Let $\eta_B= \max_{\mseq}\{\sinmaxtwo{\hat\Ab_m^{k}}\norm{\sCov}_2\}^{-1}$,
    $\sigma_m^{k_m}=\min_{\mseq}\norm{\sCov}_2$
    ,and $\kappa_{\hat a}=\max_{\mseq} \sinmaxtwo{\hat\Ab_m^{k}}/\sinmintwo{\hat\Ab_m^{k}}$.
    
    Then, $L$ iterates in Algorithm~\ref{alg:initializationB} yields
    \begin{multline*}
\norm{\Bb_i^{k,(L)}-\pBik}_F
\leq \rho^L\norm{\pBik}_F
+   \frac{C_1}{1-\rho}\frac{\eta_B}{M}\sum_{m=1}^M\norm{\hat\Ab_m^k - \pAmk}_F\\
+   \frac{C_2\eta_B}{1-\rho}
    \sqrt{\frac{s^\star k^2\log s^\star}{N}}
+
\frac{C_3\eta_B}{1-\rho}
\max_{\mseq}
    \sqrt{\frac{k_m(s^\star+1)\vee k_m(\log M + \log p+\log1/\delta_1)}{N}}
    ,
\end{multline*}
where $\rho=C(\gamma_1,\gamma_2)\cbr{1-\kappa_{\hat a}^{-1}{\nu_x}/(8\sigma_m^{k_m})}$ and  with probability at least $1-p^{-1}3\delta_0-p^{-1}\delta_1$.
\end{lemma}


==> main/8_variable_selection.tex <==
\section{Selection of Tuning Parameters}\label{sec:parameterselection}
\subsection{Selection of Basis Parameters}
%how to select basis function? how to select the number of basis functions km?
%basis selection parameter: k,km
% \kt{Emphasize that we choose $k$ both on some thresholding method}
First, we select $k_m$ based on the projection score to the basis. where we employ the elbow method to decide $k_m$ for $\mseq$. Then, we compute the canonical correlation of two views and select $k$ based on the canonical correlation score using elbow method.  The parameters $s$, $\alpha$, $\tau_1$, $\tau_2$ are selected based on $5$-fold cross validation with BIC score function:
%model selection parameter: s, alpha, tau
%K-fold cross validation with BIC?
\begin{align*}
&\BIC(s,\alpha, \tau_1,\tau_2) =
\sum_{i=1}^p\cbr{\sum_{m=1}^MN\log\det\rbr{\frac{1}{2N}\Gb_{m,i}\Gb_{m,i}^\top}
+|\hat\Nscr_i(s,\alpha, \tau_1,\tau_2)|\log N};\\
&
\Gb_{m,i}=\frac{1}{2N}\Amk \Ykmnfree{i}-\sum_{j\in\pni}\Bijk\Amk \Ykmnfree{j}.
\end{align*}


